On the Axiomatizability of Quantitative Algebras

Quantitative algebras (QAs) are algebras over metric spaces defined by quantitative equational theories as introduced by the same authors in a related paper presented at LICS 2016. These algebras provide the mathematical foundation for metric semantics of probabilistic, stochastic and other quantitative systems. This paper considers the issue of axiomatizability of QAs. We investigate the entire spectrum of types of quantitative equations that can be used to axiomatize theories: (i) simple quantitative equations; (ii) Horn clauses with no more than $c$ equations between variables as hypotheses, where $c$ is a cardinal and (iii) the most general case of Horn clauses. In each case we characterize the class of QAs and prove variety/quasivariety theorems that extend and generalize classical results from model theory for algebras and first-order structures.

==> macros.tex <==
%%%%%%%%%%%%%%%% Macros for this paper  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\qeq}[1]{=_{#1}}
\newcommand{\hb}{\overline{h}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%% Prakash's generic macros  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\newcommand{\singlespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1}\small\CS}
\newcommand{\doublespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.75}\small\CS}
\newcommand{\normalspacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{\BLS}\small\CS}
\makeatother

%       Macros for theorems (thm), propositions (prop), lemmas (lem)
%       corollaries (cor), definitions (defn), conjectures (conj),
%       remark (remark), and examples (example).
%
\theoremstyle{definition}
\newtheorem{thm}{Theorem}[section]
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{ax}{Axiom}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{fact}[thm]{Fact}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{axiom}{Axiom} 
%\newtheorem{theorem}[thm]{Theorem}
%\newtheorem{corollary}[thm]{Corollary}
%\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{defin}[thm]{Definition}
\newtheorem{df}[thm]{Definition}
%\newtheorem{definition}[thm]{Definition}
%\newtheorem{example}[thm]{Example}
\newtheorem{claim}[thm]{Claim}
\newtheorem{notn}[thm]{Notation}

\renewcommand{\l}{\langle}
\renewcommand{\r}{\rangle}

%% Generic and Logic %%
\newcommand{\pair}[2]{\mbox{$\langle #1,\; #2 \rangle$}}
\newcommand{\tuple}[1]{\mbox{$\langle #1 \rangle$}}
\newcommand{\powerset}[1]{\mbox{$\mathcal{P}(#1)$}}
\newcommand{\powfin}[1]{\mbox{$\mathcal{P}_{f}(#1)$}}
\newcommand{\ens}[1]{\mbox{$\{ #1 \}$}}
\newcommand{\alt}{\mathrel{|}}
\newcommand{\ent}{\vdash}
\newcommand{\imp}{\Rightarrow}
%\newcommand{\iff}{\Leftrightarrow}
\newcommand{\deq}{\stackrel{\rm{def}}{=}}
\newcommand{\cont}{\subseteq}
\newcommand{\iso}{\cong}                        % isomorphic ~=
\newcommand{\family}[2]{(#1)_{#2}}              % (X_n)_J or {X_n|J}
\newcommand{\rest}[1]{|_{#1}}                   % restriction S|A
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\interior}[1]{\mathaccent'27#1}
\newcommand{\bor}{\vee}
\newcommand{\band}{\wedge}

%% Lambda calculus
\newcommand{\equiva}{=_{\alpha}}
\newcommand{\redb}{\rightarrow_{\beta}}
\newcommand{\redbs}{\rightarrow_{\beta}^{*}}
\newcommand{\redn}{\rightarrow_n}
\newcommand{\redns}{\rightarrow_c^*}
\newcommand{\FV}[1]{FV(#1)}
\newcommand{\typ}{{Typ}}
\newcommand{\typedlam}{\Lambda_{\sigma}}

%% Linear Logic  %%
\newcommand{\oto}{\mathrel{\relbar\joinrel\circ}}     %Linear hom arrow 
\newcommand{\ofrom}{\mathrel{\relcirc\joinrel\relbar}}   %Lin hom back-arrow 
\newcommand{\x}{\times}
\newcommand{\os}{\oslash}
\newcommand{\oa}{\oplus}
\newcommand{\ox}{\otimes}
\newcommand{\bigox}{\bigotimes}
\newcommand{\bigoa}{\bigoplus}
\newcommand{\tadj}{\dashv}        % in-text adjunction symbol
\newcommand{\girpar}{\bindnasrempa}

%% Category theory %%
\newcommand{\set}{\mbox{$\mathbf{Set}$}}
\newcommand{\rel}{\mbox{$\mathbf{Rel}$}}
\newcommand{\mes}{\mbox{$\mathbf{Mes}$}}
\newcommand{\dom}[1]{\mathsf{dom}(#1)}
\newcommand{\cod}[1]{\mathsf{cod}(#1)}
\renewcommand{\hom}{\mathbf{Hom}}
\newcommand{\nat}{\mathbf{Nat}}
\newcommand{\vect}{\mbox{$\mathbf{Vect}$}}
\newcommand{\cat}{\mbox{$\mathbf{Cat}$}}
\newcommand{\topsp}{\mathbf{Top}}
\newcommand{\ptop}{\mathbf{Top}_{\bullet}}
\newcommand{\abgrp}{\mathbf{AbGrp}}
\newcommand{\mon}{\mathbf{Mon}}
\newcommand{\grp}{\mathbf{Grp}}



%% Analysis %%
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\nif}{\mathb{N}^{\infty}}
\newcommand{\dee}[1]{\mathrm{d}#1}

%% Modal Logic and Semantics %%
\newcommand{\may}[1]{\mbox{$\l #1\r$}}
\newcommand{\must}[1]{\mbox{$[ #1]$}}
\newcommand{\sem}[1]{\mbox{$\llbracket #1 \rrbracket$}}

%% Domain Theory %%
\newcommand{\pre}{\sqsubseteq}
\newcommand{\ua}[1]{\mbox{$\uparrow(#1)$}}    
\newcommand{\da}[1]{\mbox{$\downarrowarrow(#1)$}}    
%\newcommand{\dirsup}{\bigsqcup}
\newcommand{\dirsup}{\mathrel{\setlength{\unitlength}{.7em}\raisebox{-.2em}%
    {\begin{picture}(1,1.5)\put(.5,0){\line(-1,3){.48}}
    \put(.5,0){\vector(1,3){.5}}\end{picture}}}} % directed sup

\newcommand{\lub}{\bigvee}
\newcommand{\glb}{\bigwedge}
\newcommand{\stepfn}[2]{\mbox{$#1\nearrow #2$}}
\newcommand{\dda}{\mathord{\mbox{\makebox[0pt][l]{\raisebox{-.4ex}
                           {$\downarrow$}}$\downarrow$}}}
\newcommand{\dua}{\mathord{\mbox{\makebox[0pt][l]{\raisebox{.4ex}
                           {$\uparrow$}}$\uparrow$}}}

%% Quantum %%
\newcommand{\ket}[1]{\mathop{\big|#1\big>}\nolimits}       % |ket>
\newcommand{\bra}[1]{\mathop{\big<#1\,\big|}\nolimits}     % <bra|
\newcommand{\ketbra}[2]{\mid #1\rangle\!\langle #2 \mid}
\newcommand{\proj}[1]{\mid #1\rangle\!\langle #1 \mid}
\newcommand{\braket}[2]{\langle #1\mid#2\rangle}
\newcommand{\matel}[3]{\langle #1\mid#2\mid#3\rangle}

%% Mac Lane %%
\newcommand{\maclane}{Mac\thinspace Lane}

%% Typesetting proofs

 %      P. TAYLOR'S "END OF PROOF BOX":
 \def\pushright#1{{%            % set up
    \parfillskip=0pt            % so \par doesnt push \square to left
    \widowpenalty=10000         % so we dont break the page before \square
    \displaywidowpenalty=10000  % ditto
    \finalhyphendemerits=0      % TeXbook exercise 14.32
   %                 horizontal
    \leavevmode                 % \nobreak means lines not pages
    \unskip                     % remove previous space or glue
    \nobreak                    % don't break lines
    \hfil                       % ragged right if we spill over
    \penalty50                  % discouragement to do so
    \hskip.2em                  % ensure some space
    \null                       % anchor following \hfill
    \hfill                      % push \square to right
    {#1}                        % the end-of-proof mark (or whatever)
   %                   vertical
    \par}}                      % build paragraph
 % prefer proofs with statements, also space after
 \def\qed{\pushright{\rule{2mm}{3mm}}\penalty-700 \smallskip}

%       Robin's prf environment - modified with PT's  \qed above -
%                               - and with improved pagebreaking - 
%       For laying out a proof:  \begin{proof}{} ... \end{proof}
%       The argument is in case the proof is a continuation as in:
%           \begin{proof}{\ref{four-color} continued} ... \end{proof}
%       if you do not use the argument be careful to use the brackets!

% I have modified this to get rid of the argument.
\renewenvironment{proof}{\begin{trivlist} \item[{\bf ~Proof}.]}%
 {\qed\end{trivlist}}

% M. Barr uses the following:  "It gives a \to that can be used as
% $A\to B$ or $A\to^f B$ or $A\to^{f\o g\o h}B$ or even $A\to^f_gB$.  The
% arrow will grow to fit the label(s).  There are similar definitions for
% \two and \tofro, for which you really might want labels both above and
% below.  Actually, by reading your definition of \kto, I was able to
% simplify this.  But it is still nice to have the optional arguments.
% There is only caveat: although you can have one or the other or both
% labels, if you have both the upper must precede the lower.  These defs
% must either be placed in a style file xor surrounded by \makeatletter
% and \makeatother (but NOT both)."  (Modifications by rags)
% The definitions below look more elaborate than they need to be.
% The reason is that an empty asscript will still cause extra vertical
% spacing and the only way to avoid ugly extra space seems to be using
% some such method as this.

\makeatletter

% In-text size:

\newdimen\w@dth

\def\setw@dth#1#2{\setbox\z@\hbox{\scriptsize $#1$}\w@dth=\wd\z@
\setbox\@ne\hbox{\scriptsize $#2$}\ifnum\w@dth<\wd\@ne \w@dth=\wd\@ne \fi
\advance\w@dth by 1.2em}

\def\t@^#1_#2{\allowbreak\def\n@one{#1}\def\n@two{#2}\mathrel
{\setw@dth{#1}{#2}
\mathop{\hbox to \w@dth{\rightarrowfill}}\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\t@@^#1{\@ifnextchar_ {\t@^{#1}}{\t@^{#1}_{}}}


\def\t@left^#1_#2{\def\n@one{#1}\def\n@two{#2}\mathrel{\setw@dth{#1}{#2}
\mathop{\hbox to \w@dth{\leftarrowfill}}\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\t@@left^#1{\@ifnextchar_ {\t@left^{#1}}{\t@left^{#1}_{}}}


\def\two@^#1_#2{\def\n@one{#1}\def\n@two{#2}\mathrel{\setw@dth{#1}{#2}
\mathop{\vcenter{\hbox to \w@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \w@dth{\rightarrowfill}}%
       }\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\tw@@^#1{\@ifnextchar_ {\two@^{#1}}{\two@^{#1}_{}}}


\def\tofr@^#1_#2{\def\n@one{#1}\def\n@two{#2}\mathrel{\setw@dth{#1}{#2}
\mathop{\vcenter{\hbox to \w@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \w@dth{\leftarrowfill}}%
       }\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\t@fr@^#1{\@ifnextchar_ {\tofr@^{#1}}{\tofr@^{#1}_{}}}

% Displaysize:

\newdimen\W@dth
\def\setW@dth#1#2{\setbox\z@\hbox{$#1$}\W@dth=\wd\z@
\setbox\@ne\hbox{$#2$}\ifnum\W@dth<\wd\@ne \W@dth=\wd\@ne \fi
\advance\W@dth by 1.2em}

\def\T@^#1_#2{\allowbreak\def\N@one{#1}\def\N@two{#2}\mathrel
{\setW@dth{#1}{#2}
\mathop{\hbox to \W@dth{\rightarrowfill}}\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\T@@^#1{\@ifnextchar_ {\T@^{#1}}{\T@^{#1}_{}}}


\def\T@left^#1_#2{\def\N@one{#1}\def\N@two{#2}\mathrel{\setW@dth{#1}{#2}
\mathop{\hbox to \W@dth{\leftarrowfill}}\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\T@@left^#1{\@ifnextchar_ {\T@left^{#1}}{\T@left^{#1}_{}}}


\def\Tofr@^#1_#2{\def\N@one{#1}\def\N@two{#2}\mathrel{\setW@dth{#1}{#2}
\mathop{\vcenter{\hbox to \W@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \W@dth{\leftarrowfill}}%
       }\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\T@fr@^#1{\@ifnextchar_ {\Tofr@^{#1}}{\Tofr@^{#1}_{}}}


\def\Two@^#1_#2{\def\N@one{#1}\def\N@two{#2}\mathrel{\setW@dth{#1}{#2}
\mathop{\vcenter{\hbox to \W@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \W@dth{\rightarrowfill}}%
       }\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\Tw@@^#1{\@ifnextchar_ {\Two@^{#1}}{\Two@^{#1}_{}}}


\def\to{\@ifnextchar^ {\t@@}{\t@@^{}}}
\def\from{\@ifnextchar^ {\t@@left}{\t@@left^{}}}
\def\two{\@ifnextchar^ {\tw@@}{\tw@@^{}}}
\def\tofro{\@ifnextchar^ {\t@fr@}{\t@fr@^{}}}
\def\To{\@ifnextchar^ {\T@@}{\T@@^{}}}
\def\From{\@ifnextchar^ {\T@@left}{\T@@left^{}}}
\def\Two{\@ifnextchar^ {\Tw@@}{\Tw@@^{}}}
\def\Tofro{\@ifnextchar^ {\T@fr@}{\T@fr@^{}}}

\makeatother


\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}


\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\mfrA}{\mathfrak{A}}
\newcommand{\mfrB}{\mathfrak{B}}
\newcommand{\mfrC}{\mathfrak{C}}
\newcommand{\mfrD}{\mathfrak{D}}
\newcommand{\mfrE}{\mathfrak{E}}
\newcommand{\mfrF}{\mathfrak{F}}
\newcommand{\mfrG}{\mathfrak{G}}
\newcommand{\mfrH}{\mathfrak{H}}
\newcommand{\mfrI}{\mathfrak{I}}
\newcommand{\mfrJ}{\mathfrak{J}}
\newcommand{\mfrK}{\mathfrak{K}}
\newcommand{\mfrL}{\mathfrak{L}}
\newcommand{\mfrM}{\mathfrak{M}}
\newcommand{\mfrN}{\mathfrak{N}}
\newcommand{\mfrO}{\mathfrak{O}}
\newcommand{\mfrP}{\mathfrak{P}}
\newcommand{\mfrQ}{\mathfrak{Q}}
\newcommand{\mfrR}{\mathfrak{R}}
\newcommand{\mfrS}{\mathfrak{S}}
\newcommand{\mfrT}{\mathfrak{T}}
\newcommand{\mfrU}{\mathfrak{U}}
\newcommand{\mfrV}{\mathfrak{V}}
\newcommand{\mfrW}{\mathfrak{W}}
\newcommand{\mfrX}{\mathfrak{X}}
\newcommand{\mfrY}{\mathfrak{Y}}
\newcommand{\mfrZ}{\mathfrak{Z}}

\newcommand{\mfra}{\mathfrak{a}}
\newcommand{\mfrb}{\mathfrak{b}}
\newcommand{\mfrc}{\mathfrak{c}}
\newcommand{\mfrd}{\mathfrak{d}}
\newcommand{\mfre}{\mathfrak{e}}
\newcommand{\mfrf}{\mathfrak{f}}
\newcommand{\mfrg}{\mathfrak{g}}
\newcommand{\mfrh}{\mathfrak{h}}
\newcommand{\mfri}{\mathfrak{i}}
\newcommand{\mfrj}{\mathfrak{j}}
\newcommand{\mfrk}{\mathfrak{k}}
\newcommand{\mfrl}{\mathfrak{l}}
\newcommand{\mfrm}{\mathfrak{m}}
\newcommand{\mfrn}{\mathfrak{n}}
\newcommand{\mfro}{\mathfrak{o}}
\newcommand{\mfrp}{\mathfrak{p}}
\newcommand{\mfrq}{\mathfrak{q}}
\newcommand{\mfrr}{\mathfrak{r}}
\newcommand{\mfrs}{\mathfrak{s}}
\newcommand{\mfrt}{\mathfrak{t}}
\newcommand{\mfru}{\mathfrak{u}}
\newcommand{\mfrv}{\mathfrak{v}}
\newcommand{\mfrw}{\mathfrak{w}}
\newcommand{\mfrx}{\mathfrak{x}}
\newcommand{\mfry}{\mathfrak{y}}
\newcommand{\mfrz}{\mathfrak{z}}





